Justifiable Priority Violations

Making Deferred Acceptance more efficient requires priority violations, but which ones are justifiable? We argue that a priority can be justifiably violated if the affected student either (i) directly benefits from the improvement that caused said violation, or (ii) is unimprovable under any assignment that Pareto-dominates DA. We construct a ``just-below-cutoffs'' mechanism that always finds a justifiable DA-improvement whenever DA's outcome is inefficient, and build on it to construct an algorithm that expands justifiable improvements iteratively, converging to a matching that cannot be Pareto-improved by any justifiable outcome. Finally, we prove that both justifiability and consent frameworks have important limitations in reaching Pareto-efficient outcomes, and use data and simulations to quantify how binding these constraints are in practice.

==> difference.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Differences with Ex-Ante Consent}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As mentioned in the Introduction, there is a well-studied framework of priority violations in which waivers for priority violations (consent) is given ex-ante by students. The celebrated EADA mechanism uses this framework to generate Pareto-improvements over DA.

We conclude that justifiability offers a distinct perspective on controlled priority violations, one that admits improvements ruled out by existing frameworks.	In Example~\ref{ex:running}, this flexibility allowed us to achieve both justifiability and Pareto-efficiency simultaneously.
However, this fortunate coincidence does not hold in general.

